A unified one-shot prosody and speaker conversion system with self-supervised discrete speech units

We present a unified system to realize one-shot voice conversion (VC) on the pitch, rhythm, and speaker attributes. Existing works generally ignore the correlation between prosody and language content, leading to the degradation of naturalness in converted speech. Additionally, the lack of proper language features prevents these systems from accurately preserving language content after conversion. To address these issues, we devise a cascaded modular system leveraging self-supervised discrete speech units as language representation. These discrete units provide duration information essential for rhythm modeling. Our system first extracts utterance-level prosody and speaker representations from the raw waveform. Given the prosody representation, a prosody predictor estimates pitch, energy, and duration for each discrete unit in the utterance. A synthesizer further reconstructs speech based on the predicted prosody, speaker representation, and discrete units. Experiments show that our system outperforms previous approaches in naturalness, intelligibility, speaker transferability, and prosody transferability. Code and samples are publicly available.

==> tables/combined.tex <==
\begin{table*}[th]
  \centering
  \caption{Evaluation results for unseen speaker and prosody transfer.
  Naturalness and similarity are mean opinion scores with 95\% confidence interval.
  \textit{Topline} is a strong baseline with YourTTS~\cite{} for speaker conversion and Daft-Exprt~\cite{} for prosody transfer. Both models are with text supervision, while other methods are not. Since Daft-Exprt is not one-shot, we use source speakers from VCTK for its evaluation. \textit{GT} stands for the ground truth speech. SES is cosine similarity of speaker embedding and CER is character error rate.}
  \label{tab:main-exp}
  \centering
  \begin{tabular}{l c c c c c c c c c c}
    \toprule
    & \multicolumn{5}{c}{\textbf{Speaker Transfer}} & \multicolumn{5}{c}{\textbf{Prosody Transfer}}\\
    \cmidrule(lr){2-6} \cmidrule(lr){7-11}
    Method & CER & $f_0$-PCC & SES & Naturalness & Similarity & CER & $f_0$-PCC & SES & Naturalness & Similarity \\
    \midrule
    \textit{GT} & & & & \\
    \midrule
    \textit{Topline (text)} & & & & & & & & &\\
    \textit{SRDVC} & & & & \\
    \midrule
    \textit{Ours} & & & & \\
    \textit{Ours (vctk)} & & & & \\
    \bottomrule
  \end{tabular}
\end{table*}

==> tables/seen.tex <==
\begin{table}[th]
  \centering
  \caption{We also provide objective evaluation results of seen speakers on VCTK for comparison with SpeechSplit 2.0~\cite{SpeechSplit2} (Sp2) on three types of conversions.}
  \label{tab:main-exp}
  \centering
  \begin{tabular}{l c c c c c c}
    \toprule
    & \multicolumn{2}{c}{\textbf{Speaker}} & \multicolumn{2}{c}{\textbf{Pitch}} & \multicolumn{2}{c}{\textbf{Rhythm}}\\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
    & CER & SES & CER & $f_0$-PCC & CER & $f_0$-PCC\\
    \midrule
    \textit{Sp2} & & & & \\
    \textit{Ours} & & & & \\
    \bottomrule
  \end{tabular}
\end{table}
